Conversational Question Answering over Passages by Leveraging Word Proximity Networks

Question answering (QA) over text passages is a problem of long-standing interest in information retrieval. Recently, the conversational setting has attracted attention, where a user asks a sequence of questions to satisfy her information needs around a topic. While this setup is a natural one and similar to humans conversing with each other, it introduces two key research challenges: understanding the context left implicit by the user in follow-up questions, and dealing with ad hoc question formulations. In this work, we demonstrate CROWN (Conversational passage ranking by Reasoning Over Word Networks): an unsupervised yet effective system for conversational QA with passage responses, that supports several modes of context propagation over multiple turns. To this end, CROWN first builds a word proximity network (WPN) from large corpora to store statistically significant term co-occurrences. At answering time, passages are ranked by a combination of their similarity to the question, and coherence of query terms within: these factors are measured by reading off node and edge weights from the WPN. CROWN provides an interface that is both intuitive for end-users, and insightful for experts for reconfiguration to individual setups. CROWN was evaluated on TREC CAsT data, where it achieved above-median performance in a pool of neural methods.

==> acmart-master/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> acmart-master/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts
		


==> sections/experiments.tex <==
% !TEX root = ../2020-sigir-dp-crown.tex
\section{Experimental Setup}
\label{sec:experiments}

\subsection{Baseline and Metrics}
The provided Indri retrieval model mentioned in Section~\ref{sec:taskdescription} has been used as the baseline in our experiments.
%Maybe also use our Indri version as additional baseline?
Since responses are assessed using graded relevance,
%on a Three-Point Scale respectively five point graded relevance scale on the training respectively evaluation set, 
we used nDCG~\cite{ndcg} (normalized discounted cumulative gain) and ERR~\cite{err} (expected reciprocal rank) as metrics. Furthermore, AP (average precision) is reported on the evaluation data.
%P@1 and P@3 might also be calculated by organizers...so potentially to be included
%TODO mention qrel here?

\subsection{Configuration}

\subsubsection{Dataset.}

As mentioned in Section~\ref{sec:taskdescription}, the underlying document collection
consists of a combination of three standard TREC collections: MS MARCO, TREC CAR and Washington Post.
\subsubsection{Initialization.}
We used $word2vec$ embeddings~\cite{word2vec} pre-trained on the Google News dataset and obtained via the python library \textit{gensim}\footnote{\footnotesize{gensim: https://radimrehurek.com/gensim/}}. Furthermore, the python library \textit{spaCy}\footnote{\footnotesize{spaCy: https://spacy.io/}} has been used for tokenization and stopword removal.
As already mentioned, Indri has been used for candidate passage retrieval. We set the number of retrieved passages from Indri to 1000, so as not to lose any relevant documents.
%, since this is the maximal number of returnable passages for a query in the TREC CAsT track.
For graph processing, we used the \textit{NetworkX}\footnote{\footnotesize{NetworkX: https://networkx.github.io/}} python library. The window size $W$ for which word co-occurrences are taken into account is set to three in our graph.


\subsection{Submitted Runs}
We submitted four runs for the TREC CAsT track. These are described below.
%The underlying method is the same for each of them, however the choice of parameters differ. 
%Since CROWN is an unsupervised method, we used the training data only for tuning our parameters.

\subsubsection{Run 1: mpi-d5\_igraph (indri + graph).} 
%should the names be explained?
For our first run, we used the unweighted conversational query $cq_{1}$ and the first unweighted option $iq_{1} $  for the Indri query. 
These options performed best in our experiments. 
For definitions of $cq$ and $iq$, refer to Section~\ref{method:cq} and Section~\ref{method:iq} respectively.
The node threshold $\alpha$ is set to $0.7$, which means that nodes require having a word embedding similarity  to a query token that is greater than $0.7$ in order to influence the score calculation. The edge threshold $\beta$ is set to $0.0$ to exclude negative NPMI values. The three hyperparameters are chosen as follows:
$h_1 = 0.6$ (indri score), $h_2 = 0.3$ (node score), $h_3 = 0.1$ (edge score).


\subsubsection{Run 2: mpi-d5\_intu (indri-tuned).} 
In our second run, we vary the set of hyperparameters, while the rest stays the same as in Run 1: $h_1 = 0.9$ (indri score), $h_2 = 0.1$ (node score), $h_3 = 0.0$ (edge score). This run gives most emphasis towards the indri score, while coherence in our graph is not considered by giving no weight to the edge score.  
%give more explanaition like due to our training data which contains very limited relevance judgment this version performed better on the trainig set than run 1. However, we believe this is different on the evaluation set..? 


\subsubsection{Run 3: mpi-d5\_union (union of indri queries).} 
%In this run, the query issued to Indri is exchanged. 
Here we use $iq_{union} $ which means that we issue three separate queries to Indri and take the union of all returned passages. However, this leads to three separate Indri rankings which are incomparable. Therefore, we do not consider the indri score in our final score calculation by setting $h_1$ to $0$. Setting $h_2 = 0.6$ (node score) and  $h_3 = 0.4$ (edge score) worked best on the training data in this setting. The conversational query and the node threshold are the same as for the previous runs. 

%node_weight_threshold = 0.0
%node_similarity_threshold = 0.75 


\subsubsection{Run 4: mpi-d5\_cqw (weighted conversational query).} 
In our final run, the conversational query is varied as follows: option $cq_{2}$ is used and the node threshold is a bit more restrictive with $\alpha = 0.85$. Apart from that, the parameters are set to the same values as in Run 1.



==> sections/related-work.tex <==
% !TEX root = ../2020-sigir-dp-crown.tex
\section{Related Work}
\label{sec:related}

%Irgendwie irgendwann irgenwo~\cite{soldaini2014query}.

%Traditional models can't cope very well with conversational intents.
\textbf{Conversations in search.} 
%Answering open-domain questions can be done by traditional search engines quite well. However, they mostly cannot handle context.
Conversational questions are often posed to voice assistants. 
However, current commercial systems cannot handle conversations with incomplete context well. 
First steps to formalizing conversational search can be found in~\cite{theoreticalConvSearch}.
Furthermore, a query reformulation approach is described in~\cite{queryreformulation}: an incomplete query  is reformulated taking into account the information of previous turns in order to obtain a full-fledged query a standard search engine can deal with.
%Conversational approaches are explored theoretically in~\cite{theoreticalConvSearch}.
%Context-aware search is also considered in~\cite{searchsession1, searchsession2, searchsession3}. Information about previous queries from the same session and from click logs is used to better recognize the user's information need and thus to improve document ranking.
Apart from that, work on search sessions~\cite{searchsession1, searchsession2, searchsession3} is related to conversational search: information from previous queries from the same session and from click logs is used to better recognize the user's information need and to improve document ranking.
Further works  on search sessions focus on query suggestion by using auto-completion logs in addition to click logs~\cite{querysuggestion1, querysuggestion2}.
%Furthermore, there are approaches on query reformulation~\cite{queryreform1, queryreform2, queryreform3}.
%Since conversational queries can often be incomplete,
%TODO: maybe add further papers for query reformulation
%Some further authors tackle the conversational setting as a question completion task, like bla. -> does not consider search anymore
%add further papers for query reform..they are independent of search sessions however
However, in previous works, a ranked list of documents is usually considered as a result for a conversational query, whereas passage-level retrieval, as proposed in TREC CAsT, has not been explored yet. \\
\textbf{Conversations in reading comprehension.} 
In machine reading comprehension, answers to questions are text spans in provided paragraphs, like in the SQuAD benchmark~\cite{squad}.
%questions regarding one or several paragraphs usually need to be answered, where the answer is a text span in the provided paragraph. 
There are several benchmarks available regarding conversational reading comprehension, like QBLink~\cite{qatext1}, CoQA~\cite{qatext2}, QuAC~\cite{quac} and  ShARC~\cite{qatext3}. 
A conversational machine reading model 
%that performs very well on the ShARC benchmark 
is presented, for example, in~\cite{cmc2}. Decision rules are extracted from procedural text and reasoning is performed on whether these rules are already entailed by the conversational history or whether the information must be requested from the user.
In~\cite{cmc1} the pre-trained language model BERT~\cite{bert} is used to encode a paragraph together with each question and answer in the conversational context and the model predicts an answer based on this paragraph representation.
%TODO: maybe add further paper on methods for conversational mrc
%There is also work in the area of conversational reading comprehension where answers are text spans. 
However, these works differ from conversational search, since candidate paragraphs or candidate documents are given upfront. \\
%TODO: maybe add paper on search over tables
\textbf{Conversations over knowledge graphs.} 
Initial attempts in answering conversational questions are also being made in the area of question answering over knowledge graphs (KGs). In~\cite{saha},  the paradigm of sequential question answering over KGs is introduced and
a large benchmark, called CSQA, was created for this task.  An unsupervised approach, CONVEX, that uses a graph exploration algorithm is presented in~\cite{convex} along with another benchmark, named ConvQuestions. 
Furthermore, approaches based on semantic parsing are presented in~\cite{dialogToAction} and  in~\cite{semanticparsing}.
%an end-to-end neural model, that uses dialog memory management for inferring logical forms, is presented in~\cite{dialogToAction}.
These works differ from ours since a knowledge graph is searched for an answer, whereas in TREC CAsT large textual corpora are used as source of answer.
Questions over knowledge graphs are mainly objective and factoid, while questions over text corpora have a broader scope.
%and many of them cannot be answered by a KG because of its incompleteness.
Moreover, answers cannot always be found in KGs due to their incompleteness, whereas the required information can often be located readily in  web or news corpora.

%Therefore, the goal of the TREC CAsT track is to create a reusable benchmark for open-domain conversational search where answers are passages from text corpora. 
%also the which differ from the TREC CAsT track that a Knowledge Graph is used to answer questions.

%There are currently few datasets available in the area of  Conversational Information Seeking.
%Over KB: CSQA, ConvQuestions
%Over text: QuAC, CoQA, QBLink -> for text: MRC or Conversational RC -> passages are provided -> correct answer span needs to be detected
%Conversational search similar to work about search session -> there the focus previously have been on document retrieval. Therefore, passage-level retrieval as in this years TREC Conversational Assisstance track is still an open area. 

%Semi-structured tables from Wikipedia
%Some approaches for question completion, further approaches?


%The data collection for this track consists of a combination of three standard TREC collections: MARCO Ranking passages, Wikipedia (TREC CAR), and News (Washington Post). A ranked list of paragraphs is expected as an answer for each query. Furthermore, thirty example training topics are provided and training judgments on a three point scale (2 very relevant, 1 relevant, and 0 not relevant) are given for x topics, in total for around 120 questions, while the evaluation is performed over 50 different topics. 
%An Indri baseline using Query Likelihood is provided. For this baseline run, AllenNLP coreference resolution is performed on the query and stopwords are removed using the Indri stopword list.

%There are currently few datasets appropriate for training and evaluating models for Conversational Information Seeking (CIS). The main aim of TREC CAsT is to advance research on conversational search systems. The goal of the track is to create a reusable benchmark for open-domain information centric conversational dialogues.

%The track will run in 2019 and establish a concrete and standard collection of data with information needs to make systems directly comparable.


==> sections/results.tex <==
% !TEX root = ../2020-sigir-dp-crown.tex
\section{Results and Insights}
\label{sec:results}


\begin{center}
\begin{table}[t]
\centering
  \begin{tabular}{ |c | c | c | c | c | c| }
    \hline 
     & mpi-d5\_igraph &	mpi-d5\_intu	& mpi-d5\_union	& mpi-d5\_cqw &	indri\_baseline  \\ \hline \hline
    nDCG@1000  & 0.322 & \textbf{0.341}  &	0.195	& 0.317 &	0.293\\ \hline
    ERR@1000 & 0.147	& 0.151 &	0.038 &	0.145 &	\textbf{0.157} \\
    \hline
  \end{tabular} 
  \caption{Results on training data.}
  \label{training_results}
  \end{table}
\end{center}


%best result for run that primarily uses indri score and for err: baseline run (relevance judgments are made based on baseline retrieval -> higher agreement -> better results

%\begin{center}
%\begin{table}[t]
 % \begin{tabular}{ l |c  |c |c | c | c| c | c| c | c| c }
  %  \hline
   %  & \multicolumn{2}{c}{mpi-d5\_igraph } &	 \multicolumn{2}{|c|}{mpi-d5\_intu }	&  \multicolumn{2}{c}{mpi-d5\_union }	&  \multicolumn{2}{|c|}{mpi-d5\_cqw } &	 \multicolumn{2}{c}{median}  \\ 
    % & AP@5 & nDCG & AP@5 & nDCG & AP@5 & nDCG & AP@5 & nDCG & AP@5 & nDCG \\ \hline
     %Turn 1 & 0.0326 & 0.4971 & 0.0327 & 0.5178 & 0.0233 & 0.4438 & 0.0326 & 0.4969 & 0.0346 & 0.4721\\ \hline
     %Turn 2 & 0.0401 & 0.4475 & 0.0416 & 0.4796 & 0.0085 & 0.3295 & 0.0401 & 0.4459 & 0.0309 &  0.3666 \\ \hline
     %Turn 3 & 0.0390 & 0.4856 & 0.0396 & 0.5038 & 0.0140 & 0.3999 & 0.0385 & 0.4785 & 0.0350 & 0.4168\\ \hline
    % Turn 4 & 0.0445 & 0.4383 & 0.0518 & 0.4561 & 0.0085 & 0.3503 & 0.0458 & 0.4365 & 0.0428 &  0.3816\\ \hline
     %Turn 5 & 0.0479 & 0.4249 & 0.0533 & 0.4534 & 0.0094 & 0.3535 & 0.0510 & 0.4096 & 0.0414 & 0.3744\\  \hline
    % Turn 6 & 0.0497 & 0.4536 & 0.0593 & 0.4938 & 0.0059 & 0.3288 & 0.0506 & 0.4579 & 0.0393 & 0.3635\\ \hline
     %Turn 7 & 0.0420 & 0.4634 & 0.0513 & 0.4994 & 0.0056 & 0.3522 & 0.0425 & 0.4564 & 0.0381 & 0.4042\\ \hline
     %Turn 8 & 0.0279 & 0.3738 & 0.0318 & 0.4195 & 0.0033 & 0.2965 & 0.0254 & 0.3760 & 0.0288 & 0.3092\\\hline
     %All & 0.0391   & 0.4406 & 0.0435 & 0.4698 & 0.0096 & 0.3518 & 0.0394 & 0.4374 & 0.042 & 0.3840  \\
     
%    MAP@5  & 0.0391 & \textbf{0.0435}  &	0.0096	& 0.0394 & 0.042\\ \hline
 %   NDCG@5 & 0.2868	& \textbf{0.2964} &	0.0814 &	0.2849 &	0.296 \\ \hline
  %  NDCG@1000 & 0.4406	& \textbf{0.4698} &	0.3518 &	0.4374 & 0.384 \\
    %\hline
  %\end{tabular} 
  %\caption{Results on Evaluation Data}
 % \label{eval_results}
  %\end{table}
%\end{center}

\begin{figure}[t]
  \centering
  \begin{minipage}{.5\textwidth}
    \includegraphics[width=.5\textwidth]{images/map5.png} %our_best_median_map.png}
    \includegraphics[width=.5\textwidth]{images/ndcg1000.png} %our_best_median_ndcg1000.png}
    \end{minipage}
     \caption{Turn-wise results for our four runs on evaluation data.}
      \label{fig:turnResults}
\end{figure}




\begin{center}
\begin{table}[t]
\centering
  \begin{tabularx}{.5\textwidth}{ |l | c | *{6}{Y|} } %{ l |c  |c |c | c | c | c }
    \hline
     & mpi-d5\-\_igraph  &	 mpi-d5\_intu 	&  mpi-d5\_union 	&  mpi-d5\_cqw  &	 median & best\\ \hline \hline
     Turn 1 & 0.033 & 0.033  & 0.023  & 0.033  & 0.035 & 0.100\\ \hline
     Turn 2 & \textbf{0.040}  & \textbf{0.042}  & 0.009 & \textbf{0.040}  & 0.031 & 0.147\\ \hline
     Turn 3 & \textbf{0.039}  & \textbf{0.040}  & 0.014  & \textbf{0.038} & 0.035 & 0.128\\ \hline
     Turn 4 & \textbf{0.044}  & \textbf{0.052}  & 0.009  & \textbf{0.046}  & 0.043 &  0.141   \\ \hline
     Turn 5 & \textbf{0.048} & \textbf{0.053}  & 0.009  & \textbf{0.051} & 0.041 & 0.147 \\  \hline
     Turn 6 & \textbf{0.050} & \textbf{0.059} & 0.006  & \textbf{0.051}  & 0.039 & 0.183\\ \hline
     Turn 7 & \textbf{0.042}  & \textbf{0.051}  & 0.006  & \textbf{0.043}  & 0.038 & 0.167\\ \hline
     Turn 8 & 0.028  & \textbf{0.032}  & 0.003 & 0.025 &  0.029 & 0.205  \\\hline \hline
     All & \textbf{0.039}   & \textbf{0.043}  & 0.010 &  \textbf{0.039} & 0.034 & 0.145   \\
     
%    MAP@5  & 0.0391 & \textbf{0.0435}  &	0.0096	& 0.0394 & 0.042\\ \hline
 %   NDCG@5 & 0.2868	& \textbf{0.2964} &	0.0814 &	0.2849 &	0.296 \\ \hline
  %  NDCG@1000 & 0.4406	& \textbf{0.4698} &	0.3518 &	0.4374 & 0.384 \\
    \hline
  \end{tabularx} 
  \caption{Turn-wise results on evaluation data for AP@5. Above-median values for our submissions are in bold.}
  \label{eval_results_map}
  \begin{tabularx}{.5\textwidth}{| l| c |*{6}{Y|} } %{ l |c  |c |c | c| c | c }
    \hline
     & mpi-d5\_igraph  &	 mpi-d5\_intu 	& mpi-d5\_union	&  mpi-d5\_cqw  &	 median & best \\ \hline \hline
     Turn 1  & \textbf{0.497} & \textbf{0.518}  & 0.444  & \textbf{0.497}  & 0.472 & 0.761 \\ \hline
     Turn 2 &  \textbf{0.448}  & \textbf{0.480}  & 0.330 & \textbf{0.446} &  0.367 &  0.759 \\ \hline
     Turn 3 &  \textbf{0.486}  & \textbf{0.504}  & 0.399 & \textbf{0.479} & 0.417 & 0.779\\ \hline
     Turn 4 & \textbf{0.438} & \textbf{0.456} &  0.350  & \textbf{0.436} &  0.382 & 0.778 \\ \hline
     Turn 5 & \textbf{0.425}  & \textbf{0.453}  & 0.353  & \textbf{0.410} & 0.374 &  0.777 \\  \hline
     Turn 6 &  \textbf{0.454}  & \textbf{0.494} & 0.329 & \textbf{0.458}  & 0.364 &  0.821\\ \hline
     Turn 7 & \textbf{0.463}  & \textbf{0.499}  & 0.352 & \textbf{0.456}  & 0.404 &  0.841\\ \hline
     Turn 8 &  \textbf{0.374} & \textbf{0.420}  & 0.296 & \textbf{0.376} & 0.309 &  0.810\\\hline \hline
     All & \textbf{0.441}  & \textbf{0.470}  & 0.352  & \textbf{0.437} & 0.362 & 0.754 \\
     
%    MAP@5  & 0.0391 & \textbf{0.0435}  &	0.0096	& 0.0394 & 0.042\\ \hline
 %   NDCG@5 & 0.2868	& \textbf{0.2964} &	0.0814 &	0.2849 &	0.296 \\ \hline
  %  NDCG@1000 & 0.4406	& \textbf{0.4698} &	0.3518 &	0.4374 & 0.384 \\
    \hline
  \end{tabularx}
  \caption{Turn-wise results on evaluation data for nDCG@1000. Above-median values for our submissions are in bold.}
  \label{eval_results_ndcg}
  \end{table}
\end{center}
%\vspace*{-1.0cm}

\noindent We present the results of our four runs on the training and the evaluation data. \newline

\noindent \textbf{Training data}. We compared our runs to the Indri baseline provided by the organizers (see Table~\ref{training_results}). 
Note that for calculating the nDCG and ERR metrics for the training data, only the limited relevance judgements from the manually created conversations have been used.
Three of our runs were able to outperform the Indri baseline with respect to nDCG@1000. \newline

\noindent \textbf{Evaluation data.} In Tables~\ref{eval_results_map} and~\ref{eval_results_ndcg}, the results on the evaluation data for the metrics AP@5 and nDCG@1000 are reported. Average values for each turn (up to Turn 8) and over all turns are displayed. The results for our four runs are reported as well as the median and best turn-wise results over all submissions to the track. 
Additionally,  in Figure~\ref{fig:turnResults} the results of our four runs are visualized over eight turns for AP@5 and nDCG@1000.

There seems to be the tendency that the results increase for later turns (up to Turn 6 for AP@5) or do not vary much (up to Turn 7 for nDCG@1000). 
This means that our method is robust with respect to turn depth and that later turns successfully exploit the information available from previous turns.
%One explanation might be that later turns might benefit from the information from previous turns.
%For the best results across turns, there seems to be the tendency that the results are getting better over turns. One explanation might be that later turns might benefit from the information from previous turns.
% The results for later turns increase slightly or do not vary much for our best run and the median performance (only for Turn 8 there seems to be a drop). This means that our method is robust with respect to turn depth.
Three of our runs, namely \textit{mpi-d5\_igraph}, \textit{mpi-d5\_intu} and \textit{mpi-d5\_cqw}
achieve above-average performance with respect to both metrics.
%and also our runs \textit{igraph} and \textit{cqw} were able to reach on average or slightly above average performance. 
 %For nDCG@1000 they were clearly above average. Our expanded Indri queries for candidate retrieval seem to work well and retrieve the relevant documents. 
 %However, the re-ranking could be improved. 
 Our \textit{mpi-d5\_union} run does not achieve competitive results probably because the candidate passages which are taken from the union of the three separate Indri retrievals create a pool which is too large for effective re-ranking.



Furthermore, Table~\ref{example_snippets} shows some exemplary queries taken from the training data,  that appear at different turns in the respective conversation, together with   passage snippets taken from top-ranked passages by CROWN  (rank 1-5).
Information from previous turns is required to be able to correctly answer the questions. For example, the query ``\textit{What about in the US?}'', asked at Turn 5, needs the additional information ``\textit{physician assistants}'' and ``\textit{starting salary}'', given at Turn 1 and Turn 4 respectively. These are directly matched in the correct answer, resulting in a high node score, and additionally appear next to each other (high edge score).

\begin{center}
	\begin{table}[t]
		\centering
		\begin{tabularx}{.5\textwidth}{| c | X | X |}
			\hline
			\textbf{Turn} & \textbf{Query} & \textbf{Passage Snippet}  \\ \hline \hline
			4 & ``What makes it so addictive?'' \newline (``\textit{it}'': \textit{``smoking''}, Turn 1) & ``Nicotine, the primary psychoactive chemical in cigarettes, is highly addictive.''  
		\\ \hline
		2 & ``What makes it so unusual?'' \newline (``\textit{it}'': ``\textit{Uranus}'', Turn 1) & ``One fact that is not only unusual, but also makes Uranus markedly different from earth is the angle of its spin axis.'' \\ \hline
	3 & ``How much do Holsteins produce?'' \newline (\textit{``Holsteins''}: \textit{``cattle''}, Turn 1) \newline  (\textit{``produce''}: \textit{``milk''}, Turn 2) & ``The Holstein-Friesian is the breed of dairy cow most common in [...] , around 22 litres per day is average.''\\ \hline
	5 &	``What about  in the US?'' \newline (\textit{``about''}: \textit{``physician assistant''}, \newline Turn 1; \textit{``starting salary''}, Turn 4) & 
``Physician assistant's starting salary varies from city to city. For instance, in New York [it] is around \$69,559, [...]'' \\ \hline
9 & ``Do NPs or PAs make more?'' \newline (\textit{``NPs''}: \textit{``nurse practitioner''}, Turn 8) \newline (\textit{``PAs''}: \textit{``physician assistant''}, Turn 1)  & ``The average salary among all NPs [...] is \$94,881.22 and the average salary among all PAs [...] is \$100,497.78.''\\ 
\hline	
	\end{tabularx}
		\caption{Examples for correct answer snippets (rank 1 - 5 in CROWN) for queries from different turns taken from training conversations.}
		\label{example_snippets}
	\end{table}
\end{center}




